A Solution to Slosh-free Robot Trajectory Optimization

This paper is about fast slosh free fluid transportation. Existing approaches are either computationally heavy or only suitable for specific robots and container shapes. We model the end effector as a point mass suspended by a spherical pendulum and study the requirements for slosh free motion and the validity of the point mass model. In this approach, slosh free trajectories are generated by controlling the pendulum's pivot and simulating the motion of the point mass. We cast the trajectory optimization problem as a quadratic program; this strategy can be used to obtain valid control inputs. Through simulations and experiments on a 7 DoF Franka Emika Panda robot we validate the effectiveness of the proposed approach.

==> sol_app.tex <==
\section{Optimization Pipeline}
We now present our casade optimization strategy for the problem, first computing a task space path subject to the required higher order constraints and then obtaining the orientation trajectory based on the spill-free relationship to the acceleration, and finally optimizing the joint space motion considering the constraints of the robots.
\subsection{Task-space Spill Free Trajectory}
\subsection{Joint-space Optimization}
\begin{equation}
\begin{aligned}
\min_{w,b,\xi} \quad & \Dot{q}^{T}M(q)\Dot{q}\\
\textrm{s.t.} \quad & y_{i}(w\phi(x_{i}+b))+\xi_{i}-1\\
  &\xi\geq0    \\
\end{aligned}
\end{equation}

